Test of Time: A Benchmark for Evaluating LLMs on Temporal Reasoning

Large language models (LLMs) have showcased remarkable reasoning capabilities, yet they remain susceptible to errors, particularly in temporal reasoning tasks involving complex temporal logic. Existing research has explored LLM performance on temporal reasoning using diverse datasets and benchmarks. However, these studies often rely on real-world data that LLMs may have encountered during pre-training or employ anonymization techniques that can inadvertently introduce factual inconsistencies. In this work, we address these limitations by introducing novel synthetic datasets specifically designed to assess LLM temporal reasoning abilities in various scenarios. The diversity of question types across these datasets enables systematic investigation into the impact of the problem structure, size, question type, fact order, and other factors on LLM performance. Our findings provide valuable insights into the strengths and weaknesses of current LLMs in temporal reasoning tasks. To foster further research in this area, we are open-sourcing the datasets and evaluation framework used in our experiments: https://huggingface.co/datasets/baharef/ToT.

==> nedges_chart.tex <==
% \begin{tikzpicture}
% \begin{axis}[height=4cm,width=\linewidth,ymajorgrids=true,xmin=100,xmax=100000,ymax=1,ymin=0.88,xmode=log,legend style={at={(1,0)},anchor=south east,xlabel={Number of Training Samples (log scale)},ylabel={Accuracy}}
% ]
% \addplot[thick,color=cycle4,mark=*] coordinates {
% (100, 1.0)
% (200, 1.0)
% (500, 1.0)
% };
% \addplot[thick,color=cycle1,mark=square*] coordinates {
% (100, 0.9112902879714966)
% (200, 0.8870967626571655)
% (500, 0.9264112710952759)
% };
% \legend{Train,Test}
% \end{axis}
% \end{tikzpicture}


\pgfplotstableread{
X   Gemini GPT Sonnet
<10 82.14876033057851 76.02131438721138 58.01652892561984
10-20 68.3157894736842 62.171428571428564 56.21052631578948
>20 59.27710843373494 45.12730465320456 42.570281124497996
}\mydata

\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=10pt,
    ymin=0, ymax=100,
    ylabel={Accuracy (\%)},
    symbolic x coords={<10, 10-20, >20},
    xtick=data,
    enlarge x limits=0.3,  % Adjust this value to control spacing
    legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
]

\addplot[fill=lavender] table[x=X, y=Gemini] {\mydata}; 
\addplot[fill=chartreuse] table[x=X, y=GPT] {\mydata}; 
\addplot table[x=X, y=Sonnet] {\mydata}; 

\legend{Gemini, GPT, Sonnet}
\end{axis}
\end{tikzpicture}

==> nnodes_chart.tex <==
% \begin{tikzpicture}
% \begin{axis}[height=4cm,width=\linewidth,ymajorgrids=true,xmin=100,xmax=100000,ymax=1,ymin=0.88,xmode=log,legend style={at={(1,0)},anchor=south east,xlabel={Number of Training Samples (log scale)},ylabel={Accuracy}}
% ]
% \addplot[thick,color=cycle4,mark=*] coordinates {
% (100, 1.0)
% (200, 1.0)
% (500, 1.0)
% };
% \addplot[thick,color=cycle1,mark=square*] coordinates {
% (100, 0.9112902879714966)
% (200, 0.8870967626571655)
% (500, 0.9264112710952759)
% };
% \legend{Train,Test}
% \end{axis}
% \end{tikzpicture}

% {'10-20': , '<10': , '>20': }


\pgfplotstableread{
X   Gemini GPT Sonnet
<10 82.14876033057851 79.00826446280992 58.01652892561984
10-20 68.3157894736842 67.6842105263158 56.21052631578948
>20 59.27710843373494 54.69879518072289 42.570281124497996
}\mydata

\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=10pt,
    ymin=0, ymax=100,
    ylabel={Accuracy (\%)},
    symbolic x coords={<10, 10-20, >20},
    xtick=data,
    enlarge x limits=0.3,  % Adjust this value to control spacing
    legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
]

\addplot[fill=lavender] table[x=X, y=Gemini] {\mydata}; 
\addplot[fill=chartreuse] table[x=X, y=GPT] {\mydata}; 
\addplot table[x=X, y=Sonnet] {\mydata}; 

\legend{Gemini, GPT, Sonnet}
\end{axis}
\end{tikzpicture}
